Towards a Goal-oriented Agent-based Simulation framework for High-Performance Computing

Currently, agent-based simulation frameworks force the user to choose between simulations involving a large number of agents (at the expense of limited agent reasoning capability) or simulations including agents with increased reasoning capabilities (at the expense of a limited number of agents per simulation). This paper describes a first attempt at putting goal-oriented agents into large agent-based (micro-)simulations. We discuss a model for goal-oriented agents in High-Performance Computing (HPC) and then briefly discuss its implementation in PyCOMPSs (a library that eases the parallelisation of tasks) to build such a platform that benefits from a large number of agents with the capacity to execute complex cognitive agents.

==> sections/experiments.tex <==
In the previous chapter we have provided the implementation details of the proposed model.
We have specified the runtime execution of the simulation cycle and the agent deliberation cycle.
Also we have provided the descriptions for the most important functions and methods of the system.
Finally, we have introduced our version of HTN planner that is provided as the default means-ends reasoner in the framework.

Now we will demonstrate how our system works from the point of view of some experiments.
First, we will describe these experiments which are designed to showcase the performance metrics of the system.
Then we will introduce a real-world scenario and show how it can be implemented within our framework.

% {\color{blue}As Javier mentioned, the text at the introductions should, if possible, link to the previous chapter. Otherwise, in any case it should be adding something of value. In the case of this chapter, it would be good to point out at why we want experimentation --to be able to test the implementation in a given scenario, blah blah-- and what we want to get from it --metrics and validation of our assumptions about scaling in HPC, blah blah.}

There are two sections in this chapter: in section \ref{section:exp-structure} we outline the structure of our experiments and in section \ref{section:exp-results} we provide their results with respect to specified criteria.


\section{Structure of the experiments}\label{section:exp-structure}

In order to test the system's performance and functionality, we have designed a number of experiment sets to test different aspect of the system:

\begin{enumerate}
    \item The first set of experiments is to demonstrate the basic functionality and correctness of implementation. They demonstrate that the system runs as expected: no messages lost, no agent gets stuck for unreasonably long time in the computations and the simulation loop runs in an orderly manner for the specified number of steps. %and raw performance.
    
    \item With the second set of experiments we focus on testing the limits of the system's performance. For that we propose three numeric aspects of the simulation as parameters: the total number of agents, the total number of messages, and the size of each message, with the performance time being the metric.
    
    \item And the third set of experiments is designed to showcase the reasoning model, its expressiveness, effectiveness, and, once again, performance.
    These experiments focus on implementation of a real-world scenario.
    The most important criteria in this case is empirical: we need to ensure that the agents in the system act similarly to what would be expected of the corresponding actor in the reality.
\end{enumerate}

\subsection{Functionality tests}

In order to verify that during the runtime the system works as intended, we have designed three simple tests scenarios: \texttt{incrementation}, \texttt{ping}, \texttt{random messaging}, which involve different components of the system.

\subsubsection{\texttt{incrementation} scenario}

The scenario can be summarised as follows:

\begin{itemize}
    \item There are 3 basic agents in the simulation.
    \item Each of them uses only a simple default action block
    \item These default blocks contain only one internal action that increments the value of the agent's \texttt{counter} field
\end{itemize}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\textwidth]{images/increment.png}
    \caption{Increment scenario scheme}
    \label{fig:htn_incr}
\end{figure}

% {\color{blue}Ideally (low priority) there would be a diagram of the 3 agents, and another diagram with a sequence diagram.}

Formally, this simulation is not a MAS, as the agents do not interact, but it allows us to easily look into agents' inboxes as they are of manageable size and there are only three of them.

We expect:

\begin{itemize}
    \item The simulation to last for exactly the  specified number of round.
    \item The counter to increase uniformly and be equal to the total number of simulation steps at the end of the run.
    \item Inbox/outbox to contain only the state of the agent.
\end{itemize}


\subsubsection{\texttt{ping} scenario}

This scenario is described the following way:

\begin{itemize}
    \item There are 3 agents, the reasoning mechanism of each one based on an HTN planner
    \item The HTN used is shown on Fig.\ref{fig:htn_ping}
    \item A simple environment is used with a single field: \texttt{counter}
    \item Agents' beliefs are more complex to cover the whole range of HTN interaction; they consist of:
    \begin{itemize}
        \item boolean \texttt{got\_msgs}, denotes whether the agent has received a message
        \item integer \texttt{reply\_count}, denotes how many replies the agent has to send (note that for the testing purpose, the reply output of the \texttt{process} method is not used in this scenario)
        \item list \texttt{message}, denotes the messages the agent has received
        \item integer \texttt{counter}, used to count the number of ``pong'' messages the agent has received
        \item integer \texttt{to\_env}, denotes the value to be added to the environment's \texttt{counter}.
    \end{itemize}.
\end{itemize}

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{images/htn_ping.png}
    \caption{HTN for the ``ping'' test}
    \label{fig:htn_ping}
\end{figure}

During the simulation, each agents acts in the following way:

\begin{itemize}
    \item If the agent received a message, it processes it depending on its content:
    \begin{itemize}
        \item If it contains a ``ping'' message, the agent replies by a ``pong'' message.
        \item If it contains a ``pong'' message, it increments the environment's counter and its own counter.
    \end{itemize}
    \item If no messages were received, the agent sends a ``ping'' message to another agent that is random chosen from the directory.
    \item Once the agent's counter value is equal to 3 or more, the agent finishes its execution by sending the ``finish'' request to the controller.
    \item The ``Got Message'' method's primitive tasks' action blocks are combined together.
\end{itemize}

We expect the following results of this simulation:

\begin{itemize}
    \item The number of agents diminish until there is no more than one agent.
    \item Inboxes contain normal messages besides states.
    \item HTN logic correctly specifies the scenario instructions.
    \item Actions from the ``Got Message'' do indeed get executed as part of the same action block.
\end{itemize}


\subsubsection{Random messaging scenario}

This is the most complex of functionality tests.
The following list contains the rules of the scenario.

\begin{itemize}
    \item The simulation contains 100 agents
    \item Simulation lasts for a total of 100 steps, and is repeated 10 times.
    \item Agents' behaviors are guided by a trivial HTN with 4 actions (Fig.\ref{fig:perf_htn}):
    \begin{description}
        \item[Decide] internal action is used to randomly pick a number of messages to be sent
        \item[Send] message action is used to send the said number of messages to randomly chosen agents from the directory
        \item[Write] external action is used to send to the environment the number of messages sent and received
        \item[Cleanup] internal action is used to reset the said numbers
    \end{description}
    \item In each simulation step each agent sends from 5 to 20 messages (randomly chosen) to a random agent each, except itself.
    \item Each agent counts the number of messages it received
    \item The number of messages sent and received are written to the environment that acts as a blackboard.
    \item A special modification was made to the \texttt{agent\_step} function that counts the time it takes for each agent to finish its step.
    \item Environment's poststep writes the collected values to the log file for further analysis
\end{itemize}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{images/perf_htn.png}
    \caption{Random messaging test HTN}
    \label{fig:perf_htn}
\end{figure}

We expect the following results:

\begin{itemize}
    \item In the environment the total number of messages sent on each step is equal to the total number of messages received on the next.
    \item Agents' execution duration are approximately the same, without clear outliers
\end{itemize}


\subsection{Performance tests}

The overall time performance of the system is evaluated in accordance with the 4 parameters:

\begin{itemize}
    \item Number of agents
    \item Number of messages sent
    \item Size of messages sent (given as a number of \texttt{0} integers in the list attached to the message)
    \item Number of requested processing units
\end{itemize}

For this test cases a special simulation was designed:

\begin{itemize}
    \item Agents' behaviors are guided by a trivial HTN with a single compound task, single method, and single primitive task with 2 actions: send messages and increment step counter belief.
    \item On each turn each agent sent a specified number of messages containing lists of zeroes of specified length to random agents and incremented its ``step'' counter belief.
    \item Upon the reception of a message, each agent incremented its ``counter'' belief
    \item For each series of tests one of the parameters was modified while the others were fixed at default values.
    \item The default values were:
    \begin{itemize}
        \item Number of agents: 100
        \item Number of messages: 10
        \item Message size: 0kb
        \item Number of processes: 256
    \end{itemize}
\end{itemize}

For these tests we expect the following results:

\begin{itemize}
    \item The performance is supposed to be linearly dependent of the number of agents. Additionally, due to the fact, that all the tasks get submitted almost at the same time, we may see convex fragments between the lightly peaked points that roughly correspond to the multiples of the number of processes. This is due to the fact, that once we schedule the tasks for all the processes, the remainder will have to wait until these tasks finish, which they should do almost at the same time.
    \item Performance is expected to be sublinearly dependent of the number of messages and the size of the messages
    \item With the increase of the number of processes the performance should increase until we reach the number of processes equal to the number of agents (tasks). After that the changes are expected to be minimal.
\end{itemize}

\subsection{River-basin simulation}\label{river-sim}

One of the current real-world applications of the system is the simulation of the wastewater production and processing in the context of a river basin.
This version of the scenario is abstract, but the goal is to apply it to simulate the interactions of factories and treatment plants with the Bes\`os river in Catalonia.

In our model we represent a river as an ordered list of divisions which we call sections. Each of these sections is a 1 kilometer long part of the river. We then assume the river works in a stationary state and, therefore, each section contains a water mass that represents the mass of water that is held in that section.

We then assume water masses are characterized as: $W = \langle V, C^r\rangle$, where:

\begin{itemize}
    \item $V$ represents the volume of water
    \item $C^r$ represents pollutant concentrations and for this scenario we are only considering the following pollutant indicators: Suspended Solids (SS), Biological Oxygen Demand (BOD), Chemical Oxygen Demand (COD), Total Nitrogen (TN), and Total Phosphorus (TP).
\end{itemize}

We can then express $C^r$ as a set of the five pollutants mentioned above:
\begin{equation*}
    C^r = \langle C^1, C^2, C^3, C^4, C^5 \rangle = \langle SS, BOD, COD, TN, TP \rangle
\end{equation*}

$V$ is expressed as m$^3$ and $C^r$ are usually expressed as g/m$^3$.
\footnote{Sometimes however we express certain values in liters ($1$ m$^3$ = $1\cdot 10^3$ L) and kilograms of pollutant, which requires multiplying the concentration and volume to obtain that magnitude and then transform from grams to kilograms ($1$ Kg = $1\cdot 10^3$ g).}

The full scenario we want to simulate is composed of:
\begin{itemize}
    \item A stream-lined river with 40 sections. We assume that all of them are initialized with fresh water masses (i.e., $W=\langle 5, \langle 0,0,0,0,0\rangle\rangle$)
    \item Two Wastewater Treatment Plants (WWTPs)
    \item Two towns (households)
    \item Forty industries, divided into in the following productive sectors:
    \begin{itemize}
        \item Chemical (8)
        \item Slaughterhouse (8)
        \item Paper mill (8)
        \item Furniture plant (6)
        \item Plastics (10)
    \end{itemize}
\end{itemize}

Households and industries are the main wastewater generators in this scenario, as well as the river's headstream. 
Wastewater is considered as a water mass with significant pollutant concentrations. 
In order to maintain the water quality of the river and make sustainable use of it, Wastewater Treatment Plants handle wastewater and treat it so that it can be safely discharged into the river.
The system also contains retention tanks, which collect water when it rains and discharges it in a controlled way by laminating the water inflows into the sewer system (see Fig.\ref{fig:river}).
Some of these tanks are also used for industrial discharges.
In the following sections, each of these elements is described and specific data is provided for the simulation prototype.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{images/river.png}
    \caption{Overview of the river}
    \label{fig:river}
\end{figure}

\subsubsection{Households}

Households act as wastewater generators.
In the most realistic scenario they automatically discharge a certain volume of wastewater mass at each step; this volume and the pollutants depend on the time of the day.
For simplicity, we assume that volume and pollutant concentration does not vary along the day and households always discharge the same water mass.
However, depending on the population of each town, the characteristics of such wastewater mass will change accordingly.

For our scenario we consider two towns:

\begin{itemize}
    \item Coal Hill
    \begin{itemize}
        \item Population: 3584
        \item Location: near section 3
        \item Wastewater: $\langle 16.875, \langle 100, 130, 260, 32, 5\rangle\rangle$
    \end{itemize}
    
    \item Torchwood
    \begin{itemize}
        \item Population 27645
        \item Location: near section 36
        \item Wastewater: $\langle 130.162, \langle 200, 200, 400, 36, 7\rangle\rangle$
    \end{itemize}
\end{itemize}

Households discharge to the nearest WWTP (in terms of number of sections from the household location to the WWTP).
This discharge is done at every step.
Though the parameters of each discharge is constant for the current scenarios, we force the household agents to report the parameters of the discharge to the WWTP.

The HTN of the current version of Households is shown in Fig.\ref{fig:household_htn}.
Though the HTN in this case is trivial (and it can be replaced by the default block), we intentionally keep it as HTN for possible future scenarios.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{images/Household_HTN.png}
    \caption{HTN for Household agents}
    \label{fig:household_htn}
\end{figure}

\subsubsection{Industries}

Industries manufacture products, generating wastewater as byproduct.
We assume that these products are automatically sold and, therefore, they are instantly transformed into profit for the industries.
Also, we do not consider actual manufacturing processes and resources (like clear water) demand.
Industries have storage tanks to store the wastewater but these are limited and the wastewater has to be discharged into the sewer system (and hence to a WWTP).
However, they cannot discharge whenever they want, as explicit permission from a WWTP is required first.
In order to get such permission, industries have to pay to the WWTP the cost of treating their wastewater, so it can be discharged into the river safely (i.e. returning the water into the water cycle in a sustainable way).

An industry belongs to one of the following sectors:

\begin{itemize}
    \item Slaughterhouse
    \begin{itemize}
        \item Wastewater (per Tn produced): $\langle 1.6-6, \langle 422, 450, 986, 59, 22\rangle\rangle$
        %\item Euros per Tn produced:
        %\item Maximum production:
        \item Location: Randomly chosen between 1--40
        \item Storage capacity: 100
    \end{itemize}
    
    \item Paper mill
    \begin{itemize}
        \item Wastewater (per Tn produced): $\langle 100-250, \langle 300, 275, 580, 25, 5\rangle\rangle$
        %\item Euros per Tn produced:
        %\item Maximum production:
        \item Location: Randomly chosen between 1--40
        \item Storage capacity: 100
    \end{itemize}
    
    \item Plastics
    \begin{itemize}
        \item Wastewater (per Tn produced): $\langle 2.04, \langle350, 277, 1200, 50, 6\rangle\rangle$
        %\item Euros per Tn produced:
        %\item Maximum production:
        \item Location: Randomly chosen between 1--40
        \item Storage capacity: 100
    \end{itemize}
\end{itemize}

For simplicity, we consider that each industry type produces the wastewater following the same parameters.
Each sector has a specific pollutant concentration and a given volume (or a range of volumes).
Also, while concentrations are fixed, the tons produced by industries are not. This will respectively influence the volume of the produced wastewater (as well as the profits of the industries).
Volume depends on the number of tons produced.

The geo-location of an industry is used to determine to which exact WWTP they are connected through the sewer system (we assume they are connected always to the closest one).

Industries try to produce as much as they can at each tick but they have to see to it that:

\begin{enumerate}
    \item They are not producing more than their maximum production capacity.
    \item They are not going to produce more tons if there is a risk of overfilling the current available space in their storage tanks with byproducts.
\end{enumerate}

As it was noted at the start of this section, industries are obliged to request permissions from WWTPs to discharge their byproducts to the sewer system.
For each request, the corresponding WWTP will reply with either a refusal or a permission.
In the latter case the response will also contain the cost the industry has to pay to get its wastewater processed.
If the industry accepts, the money is detracted automatically from its account, the industry informs the WWTP about the discharge and proceeds with it (thus, also modifying its storage tanks fill status).

It is not necessary for the industry to discharge everything stored. 

The current version of an industry's HTN is shown in Fig.\ref{fig:industry_htn}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{images/Industry_HTN.png}
    \caption{HTN for Industry agents}
    \label{fig:industry_htn}
\end{figure}


\subsubsection{Wastewater Treatment Plants (WWTP)}

These plants receive wastewater inflows from the sewer system, they treat it, and then they discharge it into the river.
This reduces the pollutants concentration in the river and possibly prevents potentially harmful consequences, such as eutrophication or massive algae expansion, which would consume oxygen from the water leading to massive deaths of other living beings in the river \cite{chislock2013eutrophication}.

For our scenario we consider two WWTPs:

\begin{itemize}
    \item WWTP 1
    \begin{itemize}
        \item Location: 3
        \item Storage capacity at entrance/exit: 100/100
        \item Treatment capacity: 100
        \item Operative threshold: 0.1
        \item Pollutant treatment cost (SS/DBO/DQO/TN/TP): (200/150/150/300/300) €/kg
        \item Volume treatment cost: 100 €/m$^3$
    \end{itemize}
    
    \item WWTP 2
    \begin{itemize}
        \item Location: 36
        \item Storage capacity at entrance/exit: 100/100
        \item Treatment capacity: 100
        \item Operative threshold: 0.1
        \item Pollutant treatment cost (SS/DBO/DQO/TN/TP): (200/150/150/300/300) €/kg
        \item Volume treatment cost: 100 €/m$^3$
    \end{itemize}
\end{itemize}

In our model, wastewater arrives from different sources and its masses are merged into the WWTP entrance segment of the sewer system. 
That tank has a limit; if that limit is reached, all of the surplus wastewater is automatically bypassed to the river. 
This could happen under different circumstances:

\begin{itemize}
    \item A sudden amount of wastewater arrives because of precipitations.
    \item Industrial discharges are higher than expected.
    \item Both.
\end{itemize}

The WWTP takes some part or all of the wastewater at the entrance and moves it into the plant for treatment.
This treatment takes some time and will remove a predetermined percentage of pollutants.
The water will be kept until the process ends and, once that happens, the treated water mass will be discharged into the river section where the WWTP is located.

Additionally, the WWTP has to log the average pollutant concentrations at the entrance and exit so that a performance indicator can be computed.
Ideally, WWTPs have to keep their performance at a certain level.

Another important thing about WWTPs is that the treatment is performed with the usage of colonies of bacteria.
These colonies require nutrients obtained from the wastewater, therefore the WWTP needs a minimum flow of inflows to remain operative.
This requirement is represented by the operative threshold parameter.
It denotes the minimal fraction of a WWTP's capacity that has to be filled with wastewater (e.g., treatment capacity 10000 and operative threshold 0.1 would mean that the corresponding WWTP is required to have 1000 m$^3$ of wastewater stored at treatment at all times). 

Treating wastewater has a cost for each kilogram of pollutant extracted from the water.
This cost is different for each pollutant and is set as a model parameter.

Also, as mentioned before, treating wastewater takes some time that is expressed in terms of simulation ticks as treatment duration.
The process starts with whatever wastewater mass is at the entrance.
It then enters and is kept separated from other wastewater masses being treated for the number of ticks equal to the duration of the treatment.
After that amount of time has passed, the corresponding wastewater mass has its pollutant concentrations reduced at a given rate.
Afterwards, this wastewater mass is discharged into the river.

Besides the treatment itself and the bypassing of decisions, the WWTP has to answer requests for permissions to discharge wastewater.
It has to determine if it is feasible to accept a given wastewater discharge and at what cost according to the current load (in terms of volume and pollutant amounts that will be removed).

The WWTP estimates the price of treatment of a wastewater mass (P) as:

\begin{equation}\label{price}
    P=V_i\cdot G\cdot \mpar\sum^5_{r=1} C^r_i\cdot q^r\cdot g^r_i
\end{equation}

$q^r$ are as follows:
\begin{itemize}
    \item SS: 50 euros per kg
    \item DBO: 75 euros per kg.
    \item DQO: 75 euros per kg.
    \item TN: 120 euros per kg.
    \item TP: 150 euros per kg.
    \item Volume: 100 euros per m$^3$
\end{itemize}

It may accept wastewater mass only if $V \ge V_i$, otherwise the request is automatically rejected ($V$ here is the available storage volume in the WWTP) .

At the moment, $g^r_i$ are ignored (set to $1$) since we consider all the pollutants equally.
However, in more complex scenarios that is usually not a case as higher concentrations cause problems to the bacteria colonies in the WWTP, incurring in higher processing costs.

$G$ is a penalty factor applied by the WWTP that could be a function of the available volume (so that the WWTP increases the cost as the free storage volume is reduced).
Note that WWTP also has to try to keep a minimum storage volume available for any unexpected influents.

The HTN for WWTPs is shown in Fig.\ref{fig:wwtp_htn}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{images/WWTP_HTN.png}
    \caption{HTN for WWTP agents}
    \label{fig:wwtp_htn}
\end{figure}

\subsection{Environment}

The environment is composed of the aforementioned river, the sewer system, and of rains.
For the purpose of this scenario and for simplicity, precipitations are collected to meteorological water tank abstractions and sent to the WWTP.

Currently, we consider meteorological water tanks as part of the environment.
Therefore, meteorological wastewater is collected and then sent during the following step of the simulation.

As described in section \ref{river-sim}, the river is divided into sections of 1 km each, and we assume that it works in a stationary state. This implies that sections are defined by the watermass they hold and those masses move from one section to the following one at each simulation step.
This movement reduces pollutant concentration by a given percentage:

\begin{itemize}
    \item SS:  20%
    \item DBO: 15%
    \item DQO: 15%
    \item TN: 10%
    \item TP: 5%
\end{itemize}

When different water masses collide, they are merged using the standard chemical formulas for concentration mixing:

\begin{equation*}
    \frac{c_1 V_1 + c_2 V_2}{V_1 + V_2}
\end{equation*}

where $c_1$ and $c_2$ are concentration values, and $V_1$ and $V_2$ are the corresponding volumes of the watermasses.

Sewers are represented by parallel ``river'' segments, leading from the segments within the range of the WWTP to this WWTP.
The WWTP then perceives the wastewater at the final entrance segment and either removes it (taking it for treatment), bypasses it, or does a mix of both.

Note that water inside of the sewer system does not clean itself as the water in the river does.


\subsection{Test scenario}
For testing agents' interaction and communication in our platform, we have simplified the model by removing high-detail elements. This eases not only the task of implementation but facilitates the interpretation of the results obtained. This simplification entails not considering the rain in the proposed scenarios as well as ignoring the presence of households. Next subsections provide a thoroughly description of these scenarios

\subsubsection{One industry and one WWTP}

The scheme for these scenario is depicted in Fig.\ref{fig:scenario1}

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{images/scenario1.png}
    \caption{Scheme of the test scenario}
    \label{fig:scenario1}
\end{figure}

For the purpose of this scenario the river only has a small amount of sections (4). The industry belongs to the slaughterhouse sector:

\begin{itemize}
    \item Slaughterhouse
    \begin{itemize}
        \item Wastewater (per Tn produced): $\langle 1.6-6, \langle 422, 450, 986, 59, 22\rangle\rangle$
        \item Location: 1
        \item Storage capacity: $S_{ind}$
        \item Maximum production: $P_{ind}$ Tn/hour
        \item Euros per Tn produced: 500 \euro/Tn = B
    \end{itemize}
\end{itemize}

The WWTP discharges into the first section. 
Its details are:

\begin{itemize}
    \item WWTP
    \begin{itemize}
        \item Location: 1
        \item Treatment time: 5 hours (ticks)
        \item Storage capacity at entrance/exit: $S_{wwtp}$
        \item Treatment capacity: $S_{wwtp}\cdot$ Treatment time
        \item Treatment cost: C \euro/m$^3$
        \item Operative threshold: 0
    \end{itemize}
\end{itemize}

We also assume that there is no rain.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[height=0.7\textheight]{images/res_incr.png}
%     \caption{Output logs for the incrementation scenario}
%     \label{fig:res_incr}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \subfigure{\includegraphics[width=0.7\textwidth]{images/res_ping0.png}}
%     \subfigure{\includegraphics[width=0.7\textwidth]{images/res_ping1.png}}
%     \caption{Output logs for the ping scenario}
%     \label{fig:res_ping}
% \end{figure}

% \section{Results}\label{section:exp-results}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\textwidth]{images/ping_agent.png}
%     \caption{Agent step log for the ping scenario}
%     \label{fig:ping_agent}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \subfigure{\includegraphics[width=0.15\textwidth]{images/stat-env.png}}
%     \qquad
%     \subfigure{\includegraphics[width=0.77\textwidth]{images/stat-tasks.png}}
%     \caption{Environment values and task duration logs for random messaging scenario}
%     \label{fig:res_stat}
% \end{figure}

\subsection{Functionality tests}

The results of these tests are shown on Fig.\ref{fig:res_incr} to \ref{fig:res_stat}.
As it can be seen from the outputs, the MASs in both cases function just as expected:
% {\color{blue}What was expected?}

\begin{itemize}
    \item In the incrementation test the simulation finished after 10 iterations (numeration is from 0) with the counter value for each agent equal to 10. Moreover, there is no other messages in the agent's inboxes.
    \item For the ping scenario we see different messages in the agents' inboxes, scenario terminates when two agents is removed (leaving the system with only \texttt{Agent 1}), the removed agents have \texttt{counter} belief equal to 3.
    Fig.\ref{fig:ping_agent} shows part of a PyCOMPSs log file corresponding to one step of one agent: there we can see the planning agent's reasoning stage and also that it executes during the same step actions that are originally from different action blocks, proving the fact of their merging.
    \item For random messaging scenario we have an environment logs and task duration distribution.
    The former contains lines of numbers in form ``\texttt{messages\_sent messages\_received}'', the latter is the standard histogram with 100 bins.
    From the part of the environment log we can see that the number of the messages sent on the previous step is equal to the number of messages received on the next step.
    Simple verification script confirms the results for the whole length of the log, with expected exception of the edge cases (when there are no previous step and the next step).
    Histogram and (the range of values) show that all the tasks are executed almost instanteneously and fast, falling within the range of tens of milliseconds.
\end{itemize}


% dmitry I moved the figures 5.9 to 5.12 just before section 5.2.1 so they are printed just before this section ;-)


\subsection{Performance tests}

All of these experiments, with two exceptions, were performed on BSC NordIII cluster using in the default setting 256 processors cores per test.
Each core is Intel SandyBridge-EP E5–2670 at 2.6 GHz.
All the results are averages of 5 replications.

The time results are presented as triples of total time the test took, part of that time that was spent on task computations, and part of that time that was spent by the controller (for message forwarding and action execution).

Besides the results on the tested metrics we have obtained additional insights in the possible weaknesses of the system, and confirming the directions for the future research.
The main issue we have faced was the disk space usage.
As COMPSs transforms custom objects into files for transfer, this puts a strain on the data transfer infrastructure and may result in exceeding cluster disk memory quotas.
This has limited the scale of the results we were able to achieve (although they still exceed the standard capabilities of the non-HPC BDI platforms).
Data persistency via dataClay that we were mentioning in \S\,\ref{section:state-hpc} is the solution for the issue and we discuss it as a future research in \S\,\ref{subsec:conc-pers}.

First, we present the results for message size  in Fig.\ref{fig:res-msize}.
The message size clearly affect the performance, although the mathematical nature of this is unclear.
We assume that the ``ragged'' nature of the graph may be result of different task over nodes assignment and thus different cost of data transfer.

\begin{figure}[h]
    \centering
    \includegraphics{images/res-msize.png}
    \caption{Results for message size test}
    \label{fig:res-msize}
\end{figure}

As expected, the controller time is not affected by the size of the messages, as it only deals with the pointers to actual messages.

On the other hand, the results for message count test are clear: Fig. \ref{fig:res-mcount}. We can clearly see the sublinear dependency with increase of message numbers, although we do not have yet enough data to specify their relation beyond that.
The sublinear nature of the dependency may be explained by the fact that the messages do not take much disk space, so the most time goes for launching the transfer processes.
When all the agents get at least some messages, there is no more need to launch extra processes.

\begin{figure}[h]
    \centering
    \includegraphics{images/res-mcount.png}
    \caption{Results for message count test}
    \label{fig:res-mcount}
\end{figure}

Another observation that was expected is the noticeable increase in controller time.
As the number of messages increase, it have to forward more and more messages, which affects the performance, though still insignificantly in this scenarios.

For the number of agents the behavior of the graph (Fig.\ref{fig:res-acount}) also fits the expectations.
The graph increases linearly with increase of the total number of agents (and, correspondingly, the number of PyCOMPSs tasks).
We may also notice small convex sections that were also hypothesised although at larger scale.

\begin{figure}[h]
    \centering
    \includegraphics{images/res-acount.png}
    \caption{Results for agent count test}
    \label{fig:res-acount}
\end{figure}

Also, it is not clear enough from the plot, but the controller time also noticeably increases due to the fact that controller has to process additional messages and handle these new agents.


Probably the most exceptional results can be presented for the experiments on the number of processes, Fig.\ref{fig:res_proc}.
For them we have two graphs: for one is the graph for the default tests with specified agent behavior, the other one is for the slightly modified version of it, where on each step we have added a 1 second delay.
Both graphs start at number of processes equal to 1, and we can see that in the first case the sequential execution outperforms the distributed one.
The reason is that the distribution of tasks and infrastructure interactions take some time.
As we have explained in \S\,\ref{section:model-compss} due to that COMPSs is not suitable for fin-grained tasks.
But as soon as we imitate the harder tasks that take more time to execute, even just one second longer, the difference gets phenomenal.

\begin{figure}[h]
    \centering
    \subfigure{\includegraphics[width=0.15\textwidth]{images/res-proc0.png}}
    \qquad
    \subfigure{\includegraphics[width=0.77\textwidth]{images/res-proc1.png}}
    \caption{Results for number of processes tests. The left graph covers the case of the original agent behaviours, the right one is ones with introduced 1 second delays.}
    \label{fig:res_proc}
\end{figure}

Also notice that after the number of processes exceed the number of tasks, the changes in the computation time are almost non-existent, as COMPSs have enough resources to get all the tasks distributed with minimal delay.


\subsection{River basin simulation}

River basin have been successfully implemented and tested.
The code for the implementation is presented in the Appendix \ref{appendix:htn}.
Fig.\ref{fig:inner_river} shows the inner representation of the river that helps to facilitate easy flow of water from industries and households via sewers to WWTPs and from them and headstreams to the end of the river.
As we can see, for the case of 2 WWTPs there are essentially 3 river objects: one for the river itself, and one per sewer system connecting to each of the WWTPs.

\begin{figure}[h]
    \centering
    \includegraphics[height=0.8\textheight]{images/river_inner.png}
    \caption{Implemented representation of the river}
    \label{fig:inner_river}
\end{figure}

The HTNs were implemented as shown on the Fig. \ref{fig:household_htn}, \ref{fig:industry_htn}, \ref{fig:wwtp_htn}, with their \texttt{processing} and \texttt{perceive} functions following the scenarios guidelines:

\begin{itemize}
    \item Industries do not perceive the environment and can get the accept-proposal and reject-proposal messages from WWTPs.
    In case of the first message, it discharges the specified volume of water to the sewers (or at least as much as it can afford). In case the the second one, it marks the stored water in question as not under the question, forcing to propose its discharge once again.
    \item WWTPs perceive their entrance section of the sewers (in order to later reason about what to do with this water: bypass or store). They can receive inform messages from industries and households (which will modify their expectations of incoming wastewater), and can get the proposals from industries. In case of the latter they either refuse if they cannot accept that much wastewater, or calculate the price according to the formula \ref{price}.
\end{itemize}

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{images/river-env1.png}
    \caption{State of the river during the runtime}
    \label{fig:river_env}
\end{figure}

An example of the state of the river in textual format is shown in Fig. \ref{fig:river_env}.

As the goal of this scenario was to test the expressiveness of the system, we have successfully achieved it.
Nevertheless, the implementation of the river basin scenario in its most complex form stays as one of the main future applications of the system.



\section{Chapter summary}\label{section:exp-summary}

In this chapter we have focused on showcasing the performance of the developed system.
We have proposed experiments to provide performance evaluation of the system, as well as the ones to prove that it works as expected.
The experiments helped us to identify possible bottlenecks of the current implementation (data transfer) and, in general terms, showed that the reasoning cycle and HTN planner run correctly.

In the next and final chapter we will sum up all the work done, go over the initial list of objectives, and provide an extensive discussion of further development of the system.


==> sections/implementation.tex <==
In the previous section we introduced the agent-based simulation model and described its design features.
This section describes an instantiation of the framework in a concrete implementation.
First, we introduce the implementation of the main execution cycle, user API, and the main object classes in section \ref{section:impl-mas}, and then move on to cover the implemented reasoning tools in section \ref{section:impl-htn}.


\subsection{Multi-agent system}\label{section:impl-mas}

The whole system is implemented in Python, supporting both Python 2 and Python 3.
It is organised as a package with several modules and a list of main classes that are easily accessible by the user. These modules are:

\begin{compactdesc}
    \item[Controller]: it contains the \texttt{Controller} class, the main utility entity in the system, responsible for containing the MAS, running PyCOMPSs tasks, forwarding messages, and executing all the utility methods
    \item[Agent]: it contains the \texttt{Agent} class that is a simple container for the agent description.
    \item[Behavior]: it contains the \texttt{Behavior} class, that implicitly provides full agent's workflow; user may need to inherit their own classes from it for complex behaviours
    \item[Directory]: it contains \texttt{Directory} and \texttt{DirectoryEntry} classes that are used by the built-in directory facilitator
    \item[HTN]: contains all the HTN-related classes, as well as some of the more general ones; the full list is: \texttt{CompoundTask}, \texttt{Method}, \texttt{PrimitiveTask}, \texttt{Effect}, \texttt{Action}, \texttt{ActionBlock}, \texttt{HTNPlanner}, \texttt{BeliefSet} and \texttt{Conditions}
    \item[Messaging]: it contains \texttt{Message} and \texttt{Messagebox} classes used for agent messaging
    \item[State]: this module contains a simple \texttt{State} structure, used to transfer and work with persistent states.
\end{compactdesc}

Of all of these classes, users have direct access to (and should work directly only with): \texttt{Controller}, \texttt{BeliefSet}, \texttt{Behavior}, \texttt{ActionBlock}, \texttt{Conditions}, \texttt{Method}, \texttt{CompoundTask}, \texttt{PrimitiveTask} and \texttt{Effect}.
These classes are described in following sections, along the instructions on how to use them.

The simulation structure is defined in the Controller class and follows the scheme shown in Fig.\ref{fig:simulation}.
Essentially, a simulation run for a predefined number of steps; during each step each agent's behaviour step is marked as a PyCOMPSs task and distributed over the computation environment.
After the computations are done, their results, in form of lists of outgoing messages and actions, are collected by the controller.
Messages get forwarded to their recipients, actions get applied to the environment, and the iteration step ends, starting the next one.

\begin{figure}[!t]
    \centering
    \resizebox{.70\textwidth}{!}{\includegraphics[height=0.8\textheight]{images/simulation.png}}
    \caption{The simulation structure}
    \label{fig:simulation}
\end{figure}

This model of running the simulation was chosen on purpose to ensure the uniform flow of discrete simulated time for each agent.
Implementing and running a very basic MAS with this package is quite simple.
First of all, the user needs to create a Controller.
There is a number of options for Controller initialisation, but the simplest one does not use any parameters:
\begin{lstlisting}
from Library import Controller
controller = Controller()
\end{lstlisting}
In order to populate the system with agents, they need to be generated and registered in the Controller.
This can be done by using the Controller's \texttt{generate\_agent} method.
There are a lot of possible options, but the most basic one requires just the name specification (it may not be unique, each agent is assigned a unique identifier on generation):
\begin{lstlisting}
controller.generate\_agent("MyAgent")
\end{lstlisting}
Note, however, that this is an empty agent: it does not contain any behaviour or reasoner by default.
In order to run a simulation, the user must use the Controller's \texttt{run} method.
It takes, as input, only the requested number of iterations.
For instance:
\begin{lstlisting}
controller.run(10)
\end{lstlisting}
will run the simulation for 10 simulation steps.
However, as it was mentioned, it is an empty simulation with each agent doing nothing during its step.
In next subsections, each package module is detailed and what can be accomplished with them is shown.
Also, the agent simulation cycle is described.

\subsection{Behavior class}

The Behavior class acts as a basic template for specifying agents' behaviour.
The class itself is essentially a wrapper for several important functions: \texttt{perceive}, \texttt{process}, \texttt{goal\_check}, \texttt{reason}, \texttt{execute}, and \texttt{role\_check}\footnote{These function correspond to the functions in transition rules described in \S\,\ref{subsec:model-agents}}.
It also contains several auxiliary fields only used for temporary storage of values; they are reset at each step.

The main method in the Behavior class is \texttt{step}.
It follows the structure defined by the transition rules (see Fig.\ref{fig:mas}).

\begin{figure}[!t]
    \centering
    \resizebox{.70\textwidth}{!}{  \includegraphics[height=0.8\textheight]{images/mas.png}}
    \caption{Agent behaviour step structure}
    \label{fig:mas}
\end{figure}

At the beginning of an agent's step, its behaviour retrieves the agent's state, composed of its beliefs and the planner state.
The agent's goals $\mathbb{G}$ are represented by the state of the planner (namely, its current root) and the agent's role goals $\mathbb{RG}$ by the selected behaviour itself, as different behaviours potentially imply different implementations of various transition functions.

First of all, the agent perceives the environment.
A copy of the environment is passed to the behaviour's \texttt{perceive} method along with its beliefs, and the modified beliefs are read from its output:
\begin{lstlisting}
state.beliefs = self.perceive(environment, state.beliefs)
\end{lstlisting}
This function can be redefined by the user in a subclass.
By default, it ignores the environment and merely returns the agent's current beliefs.
The way to modify beliefs is covered in the corresponding subsection, though it can be mentioned here that you can work with the BeliefSet class quite similarly to the standard Python dictionary class (its structure is based on it).

The next stage is message processing.
The \texttt{process} function is called for each message in the agent's inbox:
\begin{lstlisting}
for message in inbox:
    state.beliefs, state.planner, reply = self.process(message, state.beliefs, state.planner)
\end{lstlisting}
This function should be redefined by the user to specify possible reactions to incoming messages.
Its inputs are: the message being processed, the agent's current beliefs, and the planner.
It must return modified beliefs, a modified planner and a reply (the latter can be set to \pynone if there is no reply).
Possible ways to modify the planner will be covered later in this subsection.
If the agent needs to send a reply to the message, it can use the \texttt{Message}'s built-in method \texttt{reply} and return its output along with the modified beliefs and planner.

After that, and following the Rule 3, the goal check is performed. Once again, the user can override this function if they might need to switch goals, otherwise the default identity function is used. This function is applied in the following way:
\begin{lstlisting}
state.planner = self.goal_check(state.beliefs, state.planner)
\end{lstlisting}
Thus, it retrieves the agent's beliefs and the planner, and returns the modified version of the latter.

Following the goal revision, the reasoning part of agent's execution is done. Here the user has two options:
\begin{compactenum}
    \item If the planner was passed as an argument to the Controller during the agent's generation, the HTN planner will be used.
    \item Otherwise, the behavior will look for a default action block that can also be passed at the agent generation (the empty action block is used by default).
\end{compactenum}
The default action block option is simple: the behaviour copies the actions in it and considers them as if they were its plan.
Otherwise, it depends on the state of the planner.
If the plan has finished or failed, the HTN will try to re-plan; otherwise, this step is skipped.

After reasoning, the agent acts upon its current plan, no matter how it was achieved.
The \texttt{execute} function is called in the following way:
\begin{lstlisting}
state.beliefs = self.execute(agent, block, state.beliefs, directory)
\end{lstlisting}
The processing of each action depends on its type and it is detailed in the following subsections.

Finally, after the execution is finished, the agent may review its role, i.e. behaviour.
A user-defined \texttt{role\_check} function is used for that purpose:
\begin{lstlisting}
role = self.role_check(state.beliefs)
\end{lstlisting}
By default, it always returns \pycom{None}.
However, if the redefined version of it returns an instance of some Behavior subclass, the corresponding request of Behavior change will be composed for the controller, and it will get changed before the next iteration of the simulation.

There are also two special fields accessible via the \texttt{self} parameter: \texttt{self.log} and \texttt{self.finished}.
The first one contains the string log to which agents may write anything.
The log gets flushed to the controller after each step and is written to a file if the user has specified one.

\texttt{self.finished} is related to a special experimental type of execution: it is possible to make each simulation step span for several execution steps.
In this case, each simulation step lasts for either a specified number of execution steps, or until all the agents set their \texttt{self.finished} flags to \pycom{True} (finished agents are excluded from the further execution in the same simulation step to optimise the load).

In the following subsections we will cover the three available types of actions.

\subsubsection{Internal actions}

The most simple action to process.
A simple one line of code is used to deal with it:
\begin{lstlisting}
beliefs = action.content(agent, beliefs, *action.args, **action.kwargs)
\end{lstlisting}
The agent object is passed in case the action requires some of the agent's descriptions.
\texttt{*args} and \texttt{**kwargs} are additional parameters the action function may require.
These parameters are used to allow for generalised functions to be passed as action functions.
For example, if one agent needs an internal action that increases belief A by 2, and the other agent needs the same action, but with an increment of 10, we may create a function that increases this belief by N using this parameter's structure and specify the N for each concrete action.

Besides just beliefs, the user can also return a ``finished'' flag (for the special case where the user defines the simulation step to span for several execution steps), and a log string that the controller will print if the user has specified a log output file.

\subsubsection{Message action}

In this case the requirements for the action function are different, as well as its expected outputs:
\begin{lstlisting}
msgs = action.content(agent, beliefs, directory, *action.args, **action.kwargs)
                for msg in msgs:
                    r, p, c, priority = msg
                    self.outbox.put(Message(sender=agent.id, receiver=r, performative=p, content=c, priority=priority))
\end{lstlisting}
So the action function for message actions should accept as parameters: the agent object, its beliefs, the directory of agents, and optional \texttt{*args} and \texttt{**kwargs} arguments.
It must return an iterable collection of tuples of the following format: \texttt{receiverID, performative, content}.

One of the important functions of messaging is the possibility to send requests to the controller.
In order to do this, the receiver should be stated as \texttt{"controller"} instead of the agent id, the performative should contain the request, and the content should contain the parameters of the request.
Here is the full list of currently supported requests:
\begin{compactdesc}
    \item[\texttt{"finished"}], no arguments: mark the agent as finished and exclude it from the simulation.
    \item[\texttt{"print"}], \texttt{\{"print": object\_to\_print\}}: request the controller to print the sent object in the standard output.
    \item[\texttt{"stop"}], no arguments: request to preemptively stop the simulation run.
    \item[\texttt{"agent"}], possible argument keys: name, behavior, beliefs, services, default\_block, planner: request generation and registration of a new agent with specified parameters (details on these can be found in the Controller subsection).
\end{compactdesc}
For messages actions, the user can also return a log string after the list of messages.

\subsubsection{External action}

Finally, the external action is a bit different from the internal and message actions.
External actions are not run during the agent's execution; instead, they are appended to the queue of outgoing actions for the controller.
Thus, they will be run by the controller itself in the following manner:
\begin{lstlisting}
self._environment = request["function"](self._environment, *args, **kwargs)
\end{lstlisting}
As it can be seen, it takes an environment and additional arguments as input and returns a modified version of the environment.

As an additional feature, the user, during the action definition (see below) of an external action, can also specify a parameter called \texttt{beliefs} (an iterable collection).
In this case, before the action is added to the outgoing action queue, the corresponding beliefs are added with their values to the \texttt{kwargs}.
This is a way to pass a belief-dependent action to the environment.

Besides the aforementioned step method, there is also an additional notable one: \texttt{initialisation}.
This method is run once for each agent at the very beginning of the simulation.
It requires an \texttt{init\_block} to be defined at the agent generation (otherwise it defaults to an empty block).
These \texttt{init\_block}s are run by this method in the same way the execution function runs the plans.

\subsection{Controller class}

The Controller is the most complex class of the whole system, as it maintains the simulation and offers a range of utility functions.

The full initialiser for the Controller has the following structure:
\begin{lstlisting}
def __init__(self, environment=None, prestep=None, poststep=None, msg_handler=None, step_limit=1, log_file=None, verbose=False):
\end{lstlisting}
During the controller initialisation, the user can specify a list of parameters: an environment, environmental pre- and poststep functions, a message handler, a step limit, a log file, and the verbosity.

The environment and the pre- and poststep functions are exactly the same as in the formalisation in \S\,\ref{subsec:model-mas}.
There are two relevant insights about the environment structure: first, it can be an instance of any class, but it must have a \texttt{copy()} method that returns its copy to be sent to agents; and second, the environment variable \textbf{must} be serialisable by the Python's \texttt{cPickle} package\footnote{Due to the way PyCOMPSs serialises objects, the user should be vigilant in order to ensure their custom objects are serialisable before using them inside of the framework (for instance, as the beliefs or the environment).
The Python's \texttt{cPickle} module is used as a serialiser; it does its job several orders of magnitude faster but with more strict constraints.
For instance, non-top-level functions are forbidden as object field values, including lambda-functions.}.
Therefore, a simple dictionary works considerably well as environment.

\texttt{log\_file} is as described in the previous sections: it specifies a file, to which the execution logs will be printed whenever there are any.
\texttt{step\_limit} is the upper bound number of execution steps for each simulation step (see the previous subsection).
Finally, \texttt{msg\_handler} is the special function that adds customisable processing of the outgoing messages.
All these messages pass through this function (identity function by default) before getting forwarded.

Though there is a lot of attributes inside the Controller class, most of them are hidden (prefixed with ``\_'').

The few public functions are setters for the environment, the pre-step and post-step, and verbosity, \texttt{get\_count()} returning the current number of agents in the simulation, and three large methods: \texttt{generate\_agent}, \texttt{register\_agent}, and \texttt{run}.

The main function among them is the \texttt{run} method that starts the simulation and controls the execution loop:
\begin{lstlisting}
run(num\_iter, performance=False):
\end{lstlisting}
It runs the simulation for \texttt{num\_iter} steps.
If the \texttt{performance} parameter is set to True, then this method will also return the performance data as a tuple formatted as \texttt{(agent\_time, controller\_time}.
The former is the total time of the simulation that was spent to compute the behavior steps, and the latter is the time spent by controller's utility functions.

Another important function that the controller provides is the agent generation.
By using it, the user does not need to explicitly deal with a number of various inner classes; rather the user just needs to pass the required parameters and they will be set and assigned automatically.
\begin{lstlisting}
generate_agent(self, name, behavior=None, beliefs=None, init_block=None, planner=None, default_block=None, services=None, register=True):
\end{lstlisting}
This method generates an agent and returns it.
Besides the aforementioned name parameter, the user may specify a custom behavior for this agent, its starting beliefs, the initialisation action block, the planner or default action block (the planner  will always take precedence), the list of the string service names of this agent for the directory facilitator, and an important boolean \texttt{register} denoting whether the generated agent should also be registered in the controller.
Most of these parameters are actually required for the registration (that is a default strategy for this method).
For pure agent generation without registering it, we would only need a name and, possibly, a behavior.
\begin{lstlisting}
register(self, agent, beliefs=None, init_block=None, planner=None, default_block=None, services=None):
\end{lstlisting}
All of the parameters, except \texttt{agent}, of this method are also optional parameters for the \texttt{generate\_agent} because of the option to simultaneously generate and register agents.

\subsubsection{PyCOMPSs tasks}

PyCOMPSs tasks form another notable part of the Controller module and, thus, they deserve a closer look.

There are two PyCOMPSs tasks present: \texttt{agent\_step} and \texttt{agent\_init\_step}, the latter being a slight alteration of the former, replacing the behavior's step method by the initialisation method.

\texttt{agent\_step} is a PyCOMPSs wrapper for the execution of a single agent.
It receives as parameters: the corresponding agent object, its inbox, the directory of agents, and the environment.
Note that there is no state in the parameters.
The reason is that as the agents are highly and inconsistently distributed, we decided to follow the paradigm of the stateless agents, i.e. their states are detached from them at the end of every step, and sent back at the beginning of the next.
This is done via the messaging mechanism.
That is where the agent's state is located in the inputs\footnote{In the future work we will explore the option of using \texttt{dataClay} framework to provide state persistence to agents. See \S\,\ref{section:conc-future}}.

The rest of the task structure is straightforward: as precaution the behaviour is sterilised of possible remnants of previous temporary data, the state is extracted from the agent's inbox, the agent behaviour's step method is invoked, the outgoing messages and actions are collected along with the renewed state, the behaviour is cleared again, and all the outgoing messages and actions are returned.


\subsection{Agent class}

The Agent class is a simple container for a few values and the corresponding agent's behaviour.
It also provides a couple of utility functions for message composition based on the ID of this agent. The Agent's fields are:

\begin{compactdesc}
    \item[\texttt{id}]: unique identifier of the agent
    \item[\texttt{name}]: string name of the agent
    \item[\texttt{behavior}]: the current behaviour of this agent
\end{compactdesc}


\subsection{BeliefSet class}\label{ss:impl-beliefset}

BeliefSet is a custom class for containing various beliefs and their values. It provides some additional functions in conjunction with other classes from the HTN module.
The basic functionality of BeliefSet if similar to the one of the standard Python dictionary type: beliefs are set in exactly the same way.
Still, there are two restrictions compared to dictionaries.
The first one is that the keys must be unique strings.
The second one is that sets and tuples cannot be used as values due to the special ways BeliefSets are dealt with by the HTN planner.
The custom class instances are possible but, in order to be used properly, they are required to have a default equality checker implemented, inequality checkers, and a hash function.


\subsection{Action and ActionBlock classes}

Action is a rather simple container for action functions.
It contains the following fields:

\begin{compactdesc}
    \item[\texttt{type}]: the string of the action type; either \texttt{"internal"}, \texttt{"external"}, or \texttt{"message"}.
    \item[\texttt{content}]: the action function. \textbf{IMPORTANT NOTE:} due to the way PyCOMPSs serialises custom objects, only top-level functions are allowed to be used as values for object fields (like Action's content).
    \item[\texttt{name}]: the name of the action for logging.
    \item[\texttt{beliefs}]: beliefs for external actions, as described above
    \item[\texttt{args, kwargs}]: additional parameters of the actions.
\end{compactdesc}

ActionBlocks are iterable containers for lists of Actions.
Besides action, they also contain the \texttt{parent} field that contains a pointer to the method that is the parent of the primitive tasks containing this block in HTN.
This is needed for block grouping during the planning.

ActionBlocks contain three important methods that users should use, designed to add actions to the ActionBlock without invoking the Action class directly:

\begin{lstlisting}
def add_internal_action(self, action, name="<action>", *args, **kwargs):
    ...
def add_external_action(self, action, name="<action>", beliefs=None, *args, **kwargs):
    ...
def add_message(self, action, name="<action>", *args, **kwargs):
    ...
\end{lstlisting}

\subsection{Directory class}

The instances of this class act as iterable containers of the information about agents.
\texttt{Directory} contains two fields for that: white pages, which is a dictionary from agent IDs to the corresponding agent entries, and yellow pages, which is a dictionary mapping all present service names to the agent entries of the agents that provide them.

Agent entries consist of the basic information to contact the agents: ID, name, and services list.


\subsection{Message class}

Although the user does not directly create Messages, they can process them in the \texttt{process} method.
The Message is a simple class, consisting of the following main fields:

\begin{compactdesc}
    \item[\texttt{sender}]: ID of the message sender
    \item[\texttt{receiver}]: ID of the message receiver
    \item[\texttt{performative}]: string of the message's performative. The proposed FIPA ACL performatives to use are \cite{fipa}:
    \begin{compactdesc}
        \item[propose:] propose to do some action
        \item[accept-proposal:] agree to a proposal
        \item[reject-proposal:] reject a proposal
        \item[inform:] provide some information
        \item[query-ff:] ask about some information
        \item[request:] ask to perform some action
        \item[agree:] agree to do some action
        \item[refuse:] refuse to do some action
    \end{compactdesc}
    \item[\texttt{content}]: the content of the message, usually, a dictionary
    \item[\texttt{priority}]: a boolean; if true, during the message processing such messages would be inserted at the beginning of the inbox, not appended to its end.
\end{compactdesc}


\subsection{HTN planner}\label{section:impl-htn}

The planner is implemented following the basic version of the planner from \cite{HTNGameAI}, as explained in \ref{section:model-reasoning}. 

The main classes are defined in the package's \texttt{HTN} module.
These classes are: \texttt{BeliefSet}, \texttt{Conditions}, \texttt{PrimitiveTask}, \texttt{Effect}, \texttt{Method}, \texttt{CompoundTask}, and \texttt{HTNPlanner}.

\subsection{BeliefSet and Conditions}

\texttt{BeliefSet} has been covered in subsection \ref{ss:impl-beliefset}.

The \texttt{Conditions} class is derived from \texttt{BeliefSet} and modifies it in a number of ways.
First of all, it can check against a \texttt{BeliefSet} object to see whether the conditions are a subset of its belief set (thus, all conditions are satisfied): \texttt{check\_conditions(\pytype, beliefs)}.
Secondly, it also accepts \pytype{tuple}s (pairs should be used, other elements will be ignored) and \pytype{set}s as special values for its beliefs.
If a belief is defined as a \pytype{tuple}, the \texttt{check\_conditions} function will check whether the corresponding \texttt{BeliefSet}'s belief value lies between the first and the second elements of this tuple.
In case of the \pytype{set}, it checks whether the belief's value is equal to one of the values in the list.


\subsection{Tasks}

\texttt{CompoundTask}s are intermediate elements in the task networks.
They do not have any actual code to be executed during the runtime, but rather contain a list of \texttt{Methods} denoting the way this task can be completed, and a parent field containing a pointer to its parent method for the HTN navigation purposes.

Each \texttt{Method} contains a \texttt{Conditions} object, a \pytype{list} of subtasks (that should be either compound or primitive), and the \texttt{parent} field.
When a planner checks a method, it tests its conditions against the planner's current belief set to see whether this method is applicable.
The methods are checked in the order of the subtasks list.
As the order is important, it is possible to specify where a new task should be inserted.

\texttt{PrimitiveTask}s are the containers for the ActionBlocks agents will try to perform.
They have a field for ActionBlock (\texttt{action\_block}, defined during the initialisation of the object and also \texttt{preconditions} and \texttt{effects} properties.

It is important to note, about the effects field of \texttt{PrimitiveTask}, that effects are quite similar to post-conditions.
They are used by planners to ``simulate'' the changes to beliefs after using this \texttt{PrimitiveTask}.
This is necessary for the sake of further planning.

\texttt{effects} is a list of instances of the \texttt{Effect} class.
Each \texttt{Effect} contains a belief name and either a string denoting the operation that should be applied to the value of this belief and the modifier value if it is used, or a function that will be applied to this belief, to simulate more complex effects.
Once again, please note that although using lambda expressions as \texttt{Effect}'s effect would have been a sound solution, COMPSs framework does not support serialisation of non-top level functions (as it is using the \texttt{cPickle} module for serialisation).

Also please note that \texttt{effects} should act exactly in the same way as actual \texttt{PrimitiveTasks}, especially in the case of heavy belief inter-dependencies. They just need to be consistent with conditions used for Methods and the PrimitiveTasks scheme.
This way, planners may not get plans as long as they could have had, and may end up with only partial plans but, after these partial plans complete, re-planning will continue the process using the actual states of the belief sets.
It is important to remember that this step is just a ``simulation'' of the plan execution. It should be faster than an actual run of the plan.
It is entirely up to the user to find the balance between the complexity of the planning effects simulation and the plans length.


\subsection{Planner}

As it was explained in Section \ref{section:model-reasoning}, the \texttt{HTNPlanner} is based on the hierarchy of tasks.
It starts with a root compound task and a copy of the current set of beliefs and expands via \texttt{CompoundTask}s' \texttt{Method}s and \texttt{Method}s' subtasks.
During an iteration of reasoning, a planner traverses the graph once, following a depth-first policy.
During the search, it maintains a stack of tasks to process.
When the planner processes a \texttt{CompoundTask}, it checks the conditions of its methods one by one in the order defined by the user during the methods insertion.
The first \texttt{Method} whose conditions are satisfied by the current beliefs is selected.
If no method is applicable, the planner rolls back to the previous unprocessed task undoing the changes to the current plan if there were any (if it was checking the root, it returns the current plan).
The selected method's subtasks list is added to the top of the stack of tasks to process (in the original order).

When the planner processes the \texttt{PrimitiveTaks}, it also checks it preconditions.
If they are satisfied, this \texttt{PrimitiveTask} is added to the current plan and its \texttt{Effect}s are applied in order to the current version of the simulated belief set.
If they are not satisfied, the planner rolls back.


\subsection{Implementing custom HTN}\label{subsub:customhtn}

To make use of the HTN planner, users need to define the HTN and create an \texttt{HTNPlanner} object based on it.
Some examples of the HTNs and their representation in the form of code is given in the appendix \ref{appendix:htn}.

\texttt{CompoundTask}'s constructor: 
\begin{lstlisting}
def __init__(self, methods=None, name=""):
\end{lstlisting}
It is possible to pass no arguments during the initialisation and insert (or remove) the methods later via \texttt{add\_method(value, index=\pynone)} and \texttt{remove\_method(index)} methods.
Name is an optional field that can be used to display the understandable task name in the verbose mode (note that as planning happens in the corresponding task nodes in COMPSs, this planner runtime description is outputted to the corresponding job's \texttt{.out} files).

\texttt{Method}'s constructor
\begin{lstlisting}
def __init__(self, conditions, subtasks=None, append=False, name=""):
\end{lstlisting}
\texttt{Condition}s must be passed as an argument during the initialisation. Subtasks may be added later in the same way the methods may be added to \texttt{CompoundTask}s: \texttt{add\_subtask(value, index=\pynone)}, \texttt{remove\_subtasks(index)}.

\texttt{PrimitiveTask}'s constructor:
\begin{lstlisting}
def __init__(self, name, preconditions, effects=None, action_block=None):
\end{lstlisting}
\begin{compactdesc}
    \item[\texttt{name}] is a string used in the verbose mode.
    \item[\texttt{preconditions}] is a \texttt{Conditions} object.
    \item[\texttt{effects}] is a list of Effects \item[\texttt{action\_block}] is the block of action corresponding to the task.
\end{compactdesc}

\texttt{Effect}'s constructor:
\begin{lstlisting}
def __init__(self, belief=None, effect="add", value=None):
\end{lstlisting}
\begin{compactdesc}
    \item[\texttt{belief}] is the name of the belief to modify.
    \item[\texttt{effect}] is either a string denoting the operation to be performed or the function to be applied; the function should accept beliefs as an input and return modified beliefs as an output.
    \item[\texttt{value}] is the modifier's value (if applicable).
\end{compactdesc}

The list of the supported \texttt{effect} actions and the corresponding operations:
\begin{compactdesc}
    \item[\texttt{add}/\texttt{sub}]: addition / substraction
    \item[\texttt{mul}/\texttt{div}]: multiplication / division
    \item[\texttt{mod}]: modulus
    \item[\texttt{pow}]: power
    \item[\texttt{rep}]: reassignment
    \item[\texttt{and}/\texttt{or}/\texttt{not}]: logical AND / OR / NOT
\end{compactdesc}

\texttt{BeliefSet}'s and \texttt{Conditions}'s constructors:
\begin{lstlisting}
def __init__(self, beliefs=None):
\end{lstlisting}
\texttt{beliefs} must be passed as a dictionary. If nothing is passed, an empty dictionary is created.

\texttt{HTNPlanner}'s constructor:
\begin{lstlisting}
def __init__(self, root_task, verbose=False):
\end{lstlisting}
The user just needs to pass the top level compound task (as \texttt{root\_task}) as all the network is reachable from it.
If \texttt{verbose} is \pycom{True}, the planner will generate a short summary of the current step and, in case of re-planning, the jobs will also contain the trace of this process.

Re-planning is made by invoking the \texttt{planner.replan(beliefs)} method.
It clears the current plan, and starts the breadth-first decomposition of the HTN, beginning by the root compound task.
Each method of this compound task is checked and the first one the conditions of which are satisfied is selected.
The sub-tasks of the selected method are added to the queue of tasks to check.
When an element is dequeued, what happens next depends on its type: if it is a compound task, the procedure is the same as with the root task; otherwise, if it is a primitive task, its preconditions are checked and if they are satisfied, this primitive task's action block is added to the plan.
As an additional feature, it is possible to set \texttt{method.append} to \pycom{True}.
In this case, the action blocks of all the child tasks of this method (to the very bottom of the HTN tree) will be put together in one action block.

The planner automatically follows the generated plan block by block. All that agents need to do is to call \texttt{planner.next\_block()} to get the next action block of the plan (this is done once per \texttt{agent\_step} as specified in the Behavior description).


\subsection{Limitations and possible improvements}\label{section:impl-lim}

As the framework implementation is still a raw prototype, various things may be improved from the implementation point of view.

First of all, a sophisticated logging system is needed.
As of now, the user is responsible of either directly writing to files from the external action and pre- or post-step functions.
A universal logging system based on the current log objects may be implemented and optimised.

Besides the logs, the framework might benefit from additional goal types, thus enhancing the capabilities of the planner and the possible complexity of the simulation.

Although now the environment can be assigned as any object, it makes sense from the formalisation and data persistence point of view to create a predefined structure for the purpose.
Moreover that will allow us to introduce the concept of agent scopes: as the environment can be huge and not fully observable, it makes sense to send to agents, or provide them, only the specified part of it.

==> sections/results.tex <==
In the previous section we introduced the agent-based simulation model and described its design features.
This section describes an instantiation of the framework in a concrete implementation and provides some preliminary test results.
First, we briefly describe the main points of the model implementation in section~\ref{section:impl-mas}, and then move on to cover the use of the model for a real world scenario in section~\ref{section:river-sim}.

\subsection{Implementation}\label{section:impl-mas}
The whole system is implemented in Python, supporting both Python 2 and Python 3.
It is organised as a package with several modules and a list of main classes that are easily accessible by the user:
\begin{compactdesc}
    \item[Controller:] defines the \texttt{Controller} class, the main utility entity in the system, responsible for containing the MAS, running PyCOMPSs tasks, forwarding messages, and executing all the utility methods
    \item[Agent:] defines the \texttt{Agent} class that is a container for the agent description.
    \item[Behavior:] defines the \texttt{Behavior} class, that implicitly provides the agent's workflow; user may subclass this for complex behaviours
    \item[Directory:] defines \texttt{Directory} and \texttt{DirectoryEntry} classes that are used by the built-in directory facilitator
    \item[HTN:] defines all the HTN-related classes, as well as some related functioality; the full list is: \texttt{CompoundTask}, \texttt{Method}, \texttt{PrimitiveTask}, \texttt{Effect}, \texttt{Action}, \texttt{ActionBlock}, \texttt{HTNPlanner}, \texttt{BeliefSet} and \texttt{Conditions}
    \item[Messaging:] defines \texttt{Message} and \texttt{Messagebox} classes used for agent messaging
    \item[State:] defines the \texttt{State} structure, used to transfer and work with persistent states.
\end{compactdesc}

The \texttt{Behavior} class follows the model presented in \ref{subsec:model-agents} with its instance functions corresponding to the functions in rules.
In complex scenarios it is expected that user redefines the following functions (as used in code):
\begin{lstlisting}
state.beliefs = self.perceive(environment, state.beliefs)
for message in inbox:
    state.beliefs, state.planner, reply = self.process(message, state.beliefs, state.planner)
state.planner = self.goal_check(state.beliefs, state.planner)
role = self.role_check(state.beliefs)
\end{lstlisting}

A simulation is run by initializing a Controller object, registering agents with it, and calling the \texttt{run} method.
An example of the latter two:
\begin{lstlisting}
controller.generate_agent("Test agent", behavior=MyBehavior(), beliefs=myBeliefs, init_block=None, planner=myPlanner, default_block=None, services=["testing"], register=True)
controller.run(num_iter=10, performance=False)
\end{lstlisting}

An HTN planner can be generated following the structure defined in \ref{section:model-reasoning}.
User needs to create a structure of \texttt{PrimitiveTask}s, \texttt{Method}s, and \texttt{CompoundTask}s and use the root \texttt{CompoundTask} as a parameter for the planner's initialization.

Tests showed linear performance dependency on the number of agents, sublinear on the message size and message count.
Also, performance improves drastically when the number of agents is less than the number of available nodes.


\subsection{River-basin simulation}\label{section:river-sim}

To demonstrate how the proposed model can be applied to real world problems we have implemented a scenario of pollution and wastewater distribution and treatment for the Bes\`os river in Catalonia \cite{Gomez-Sebastia2017}.
This version of the scenario is abstract, but the ultimate goal is to apply the model to simulate the interactions of factories and treatment plants at a high level of detail.

In our model we represent an environment (i.e. a river) as an ordered list of divisions which we call sections.
Each section contains a water mass that represents the mass of water that is held in that section.
Each water mass is a tuple of volume of water (V) in m$^3$ and concentration values of five different pollutants in g/m$^3$: Suspended Solids (SS), Biological Oxygen Demand (BOD), Chemical Oxygen Demand (COD), Total Nitrogen (TN), and Total Phosphorus (TP).

This agent-based simulation comprises three types of agents: households, industries, and wastewater treatment plants.
Households and industries are the main wastewater generators in this scenario. 
Wastewater treatment plants handle wastewater and treat it so that it can be safely discharged into the river.
The system also contains retention tanks, which collect water when it rains and gradually discharges it % in a controlled way by laminating\jnote{wrong verb, I'm sure} the water inflows
into the sewer system. Industries also have storage tanks to manage their own wastewater discharges.
In our simulation we defined an HTN for each type of agent (see~Fig.\ref{fig:industry_htn} for an example). 
%The current version of the industry HTN is shown in~Fig.\ref{fig:industry_htn}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.75\textwidth]{images/Industry_HTN.png}
    \caption{HTN for Industry agents}
    \label{fig:industry_htn}
\end{figure}

The HTNs are implemented with their \texttt{processing} and \texttt{perceive} functions following the scenarios guidelines:
\begin{compactenum}
    \item Industries do not perceive the environment but receive accept-proposal and reject-proposal messages from WWTPs.
    In case of the first message, it discharges the specified volume of water to the sewers (or at least as much as it can afford). In case of the second, it marks the stored water in question as not dischargeable, forcing to propose its discharge again later.
    \item WWTPs perceive their entrance section of the sewers to decide if the water can be treated with current available space or it has to be passed directly into the river. They can receive inform messages from industries and households, which will modify their expectations of incoming wastewater, and can receive proposals from industries. In the latter case, they either refuse if they cannot accept that much wastewater, or calculate a price to treat it.
\end{compactenum}
Some simulation outputs are demonstrated in Figs.~\ref{fig:sim-water} and~\ref{fig:sim-budget}.
In this simple scenario we have a 100 industries and 2 WWTPs.
Each industry produces a varying amount of wastewater at each time step depending on the amount of storage available (limited to 100~m$^3$) and immediately asks permission to discharge it; WWTP treatment takes 5 time steps to complete, then discharges it into the river.
Additionally, WWTPs have limited entrance storage space.

From Fig.~\ref{fig:sim-water} we can see the effects of limited WWTP entrance storage on industries' production: they are allowed to discharge less wastewater than they can produce which leads to full storages for all time steps after the beginning.
Periodic behaviour of discharge volumes are due to the time lag of the messaging and the fact that all of the industries start at the same time step: essentially, they ask to discharge what wastewater they have, after which they are forced to wait for the response before they can produce some new water mass or ask again about the stored one.
Note that time step 3 is the first when industry is allowed to discharge.
Periodic discharges also have visible effect in Fig~\ref{fig:sim-budget}, as industries cannot produce new goods when their storages are full.

\begin{figure}[!t]
    \begin{subfigure}[b]{0.526\textwidth}
    \includegraphics[width=0.95\textwidth]{images/sim-water.png}
    \caption{Average wastewater volumes}
    \label{fig:sim-water}
    \end{subfigure}\hfill%
    \begin{subfigure}[b]{0.474\textwidth}
    \includegraphics[width=0.95\textwidth]{images/sim-budget.png}
    \caption{Average industry profit}
    \label{fig:sim-budget}
    \end{subfigure}
    \caption{Simulation outputs}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../CCIA"
%%% End:

